Probing Image Compression For Class-Incremental Learning

Image compression emerges as a pivotal tool in the efficient handling and transmission of digital images. Its ability to substantially reduce file size not only facilitates enhanced data storage capacity but also potentially brings advantages to the development of continual machine learning (ML) systems, which learn new knowledge incrementally from sequential data. Continual ML systems often rely on storing representative samples, also known as exemplars, within a limited memory constraint to maintain the performance on previously learned data. These methods are known as memory replay-based algorithms and have proven effective at mitigating the detrimental effects of catastrophic forgetting. Nonetheless, the limited memory buffer size often falls short of adequately representing the entire data distribution. In this paper, we explore the use of image compression as a strategy to enhance the buffer's capacity, thereby increasing exemplar diversity. However, directly using compressed exemplars introduces domain shift during continual ML, marked by a discrepancy between compressed training data and uncompressed testing data. Additionally, it is essential to determine the appropriate compression algorithm and select the most effective rate for continual ML systems to balance the trade-off between exemplar quality and quantity. To this end, we introduce a new framework to incorporate image compression for continual ML including a pre-processing data compression step and an efficient compression rate/algorithm selection method. We conduct extensive experiments on CIFAR-100 and ImageNet datasets and show that our method significantly improves image classification accuracy in continual ML settings.

==> sections/02_Related.tex <==
\section{Background and Related Works}
\label{sec:related}
% \subsection{Class-Incremental Learning with Compression}
In class-incremental learning (CIL), training data are presented in sequence, and in each step, the model will encounter new incoming class data for training. During testing, the model's performance is evaluated based on the overall accuracy among both previously seen classes and new incoming classes. Consequently, an effective incremental learning model must strike a balance between preserving learned patterns from prior tasks and capturing the characteristics of new tasks. This is also referred to as the stability-plasticity dilemma~\cite{Stability_Plasticity}, where 'stability' denotes the preservation of prior knowledge, and 'plasticity' signifies the adaptation to new knowledge. Recent works on memory replay-based approaches have begun to focus on reducing the memory required per image, with the help of compression~\cite{Wang2022MemoryRW, CIM_CIL}. \textcolor{red}{However,} In our work, instead of designing a specific compression algorithms as in the previous work ~\cite{CIM_CIL}, we aim for a general method that can work for various compression algorithms in a plug-and-play manner. We examine various image compression methods on both uncompressed datasets and compressed datasets and proposed a straightforward plug-in method for incremental learning that leverages the benefits of compression.

\subsection{Image Compression}
% - Image compression is a well-known technique.
% - Lossless compression such as PNG~\cite{boutell1997png}.
% - Traditional, hand-crafted lossy image compression methods such as JPEG~\cite{wallace1992jpeg}, JPEG 2000~\cite{Skodras2001jpeg2000}, and WebP.
% - Recently, learning-based lossy image compression method: compressive autoencoder~\cite{balle2016end2end}, the Hyperprior model~\cite{balle18hyperprior}, and its improved versions~\cite{minnen2018joint, yang2020improving}.

% Image compression is an important technique in data communication and storage.
Image compression methods are broadly classified into lossless and lossy techniques.
Lossless compression algorithms such as PNG~\cite{boutell1997png} compress data by exploring the statistical redundancy of data in a way that the exact original data can be reconstructed from the bitstream.
In contrast, lossy compression methods achieve even lower bit rates by allowing a certain amount of distortion.
This category includes traditional, hand-crafted methods such as JPEG~\cite{wallace1992jpeg}, JPEG 2000~\cite{Skodras2001jpeg2000}, and WebP.

More recently, the development of learning-based lossy image compression has introduced many new methods to the field.
Most existing methods are based on the compressive autoencoder framework~\cite{balle2016end2end, theis2017lossy}.
% The Hyperprior model~\cite{balle18hyperprior} introduces a hierarchical entropy model that significantly improves the lossy image compression performance.
Notably, the Hyperprior model~\cite{balle18hyperprior}, which introduced a hierarchical entropy model, has significantly boosted the performance of lossy image compression.
% This model was subsequently refined and enhanced in several works~\cite{minnen2018joint, yang2020improving}.
Subsequent works~\cite{minnen2018joint, yang2020improving} have further improved this model, demonstrating the potential of learning-based approaches.



